The TESTMED Project Experience. Process-aware Enactment of Clinical Guidelines through Multimodal Interfaces

Healthcare is one of the largest business segments in the world and is a critical area for future growth. In order to ensure efficient access to medical and patient-related information, hospitals have invested heavily in improving clinical mobile technologies and spread their use among doctors. Notwithstanding the benefits of mobile technologies towards a more efficient and personalized delivery of care procedures, there are also indications that their use may have a negative impact on patient-centeredness and often places many cognitive and physical demands on doctors, making them prone to make medical errors. To tackle this issue, in this paper we present the main outcomes of the project TESTMED, which aimed at realizing a clinical system that provides operational support to doctors using mobile technologies for delivering care to patients, in a bid to minimize medical errors. The system exploits concepts from Business Process Management on how to manage a specific class of care procedures, called clinical guidelines, and how to support their execution and mobile orchestration among doctors. As a viable solution for doctors' interaction with the system, we investigated the use of vocal and touch interfaces. User evaluation results indicate a good usability of the system.

==> vocal_interfaces.tex <==
\subsection{Vocal Interfaces}
\label{subsec:vocal_interfaces}

Computer input interfaces have been evolving to provide humans with the most satisfying user experience. The guiding factor in this evolution is providing interfaces that correspond to all human senses (with more emphasis given to visual, verbal, and tactile interaction), which in turn brings a more relaistic dialog between the human and the computer. With the availability of smart mobile devices (which have become smaller and more powerful), the call for new computationally effective interfaces besides the traditional ones(i.e., HD displays and multitouch screens) rises up. This demand on providing a more natural feasible interaction is becoming higher, and there are many recent research work discuss the limitations and the oppurtunities, starting from introducing the integrate pen and the speech input, to the use of computer vision and image processing for providing a better visual interaction by integrated cameras. These new methodolgies shed light on the importance of multimodal interaction. Particualrly, this discusses the possibility of performing the same tasks using different interaction techniques considering to provide target users with the interaction models that best support them in accomplishing these tasks.

Vocal interfaces emerged in the new technology as many recent works disscussed their necessity. \cite{marx2001system} developed a patent work of interactive speech applications in telephone systems, where interactive dialog tasks whith users (i.e., callers) can be predefined as dialog modules to be accomplished according to user verbal-input command. In smart mobile devices, the need of applying multimodal interface that provides a vocal interaction is becoming essential, as their display screens are realtively small and vocal input would be easier, faster and more efficient to perform tasks if compared with the usual touch interface. This was indicated by the work of \cite{hedin2001voice}, where they suggested to use voice-controlled interface with smart mobile devices that are used as smaller terminals than the traditional PC ones to remotely control service applications, which can help to overcome the disadvantages of reading large amounts of text(e.g., selection menus) and typing in response on small touch keyboard. Another work of \cite{ativanichayaphong2012dynamically} discussed the use of speech recognition vocabularies that are supported by VoiceXML to dynamically generate a vocal help prompt in a multimodal applications deployed on multimodal web browsers. Additionally, \cite{sharma2003speech} considered the case of crisis management and suggested that providing multimodal interfaces whith vocal interaction feature would be highly valuable in such environment, which can definitely lead to solve issues in shorter time and ensures better collaboration among team members. To that extent, \cite{potamianos2004audio} questioned the automatic speech recognition (ASR) performance and argued the required level for speech to become a truley pervasive user interface. They added that "visual speech" (where speech recognition is supported by visual supplement) is considered the most promising source of providing additional speech information; as it clearly assists providing clear context of voice detection while locating the audio source (speaker), sustains the audio by adding speech segmental information (relating to phonetic segments of the analysed speech; i.e., words), and serve to identify the place of articulation. On the other hand, Mori \cite{Mori:2003:TSD:604045.604069} in his work of nomadic applications with multiplatform user interfaces suggested using a new methodology based on multiple abstractions to make it easier for both designers and developers of such system. Due to the importance of vocal interaction in such multidevice user interface, Paterno's suggested methodology together with the used tool support the design and development of vocal interfaces for various platforms.

Recently, many commercial prototypes of vocal interfaces were introduced in the industry. This can be easily noticed in many mobile systems, where vocal interface (as a natural language user interface) is provided to serve as an intelligent personal assistant and knowledge navigator. Such systems include \textbf{Siri}, whcih is a computer program developed by Apple Inc. as part of its operating system (i.e., iOS). This program \emph{listens} to user vocal input and interrupts it as verbal commands using Artificial Intelligence (AI) then it responds vocally back to user after analysis and accordingly to imitate human-to-human vocal interaction. A similar system called \textbf{Cortana} was founded by Microsoft and presented as a digital agent that assists users to complete tasks. Google, moreover, is competing with its newly developed system \textbf{Google Now} that provides the same idea of a vocal interface to answer questions, make recommendations, and perform actions by delegating requests to a set of web services. Google's proposed system not only answers users' queries, but also predicts what addtional information they may want based on their search history. These systems together with others like Amazon Alexa, Samsung's S Voice, and BlackBerry's Assistant show live examples of how vocal interfaces can actively help performing tasks or services for an individual with more natural interaction. On the other hand, \cite{doi:10.1001/jamainternmed.2016.0400} in their study in JAMA Internal Medicine found that Siri and similar intelligent personal assistants often gave unhelpful responses to mental health questions.

In health systems, vocal interfaces were importantly introduced in various applications. \cite{hansen2005using} suggested using vocal input to detect the fall of elderly persons who live alone, where the system is implemented on a mobile device and is attached to an accelerometer to help identifying a suspected fall and asks for an immediate response vocally, where using keypad typing could be impractical in such critical situation. In the direction of tele-home health care,
\cite{Lisetti2003245} examined the voice input as a source for representing patients' emotions while being monitored remotely, which even needs high level of skills, professionality, and competence while being counducted in person. They pointed that detecting patients' emotions vocally could be even more accurate as patiens themselves find difficulties to express precisely their own state of feeling, and therefore emphisized the importance of developing such multimodal intelligent affective interfaces. A similar work was conducted in the field of psychopathology \cite{cohn2009detecting}, where clinical diagnosis of major depression cases were applied using facial actions and vocal prosody to help automatic detection of depression, whose assessment could almost entirely depend on verbal report(e.g., during clinical interview or through questionnaire). Another work discussed the involvment of Robots in healthcare systems (e.g., hospitals), where \cite{mumolo2001pro} proposed applying vocal interaction with the service mobile Robots around the healthcare center for better and efficient realization of tasks in such ambience. This vocal interface is supported by NLP (i.e., Natural Language Processing) and supported by prosody-based dialogue modelling (i.e., grouping of sentences according to several patterns and segments). In their work of presenting multimodal integration of continuous spoken language and continuous gesture, \cite{Cohen:1997:QMI:266180.266328} included in his prototype an example of medical informatics in which users (patients in this case) can search using speech and gesture for available healthcare providers on a map in their zone. The multimodal input in this prototype is then translated into a query that is triggered on the database of all healthcare providers (e.g., doctors) in the selected area, and retrieve back results which can be then showed directly on the map. Towards establishing a health smart home that serves as an ambient intelligent space which supports eldery and those with special needs to conducts every-day life activities, \cite{Fleury2013} argued employing audio interfaces to help this group of people to easily interact with such smart environment as it doesn't require any attachment to some devices or be phisically available near any system's artifact (which in both cases could be most likely impractical). In a different scenario, he added that such system could enhance security awareness for any possible accident to happen (e.g., eldery people could use a voice command to turn on lights at night which could prevent a potential fall). Regarding the navigational assistance for surgical interventions, \cite{billinghurst1996expert} developed a prototype which uses virtual reality concept with multimodal interface (including vocal input) together with an expert system that helps to infer context in order to provide support for surgeons, either in a simulation procees or in a realistic intervention, and for both training and clinical purposes.

Up to this point, vocal interfaces in a multimodal interactive applications have been employed in healthcare research. Recently, many research activities related to healthcare have focused on supporting giudlines modeling and process management in static and well defined clincal contexts and healthcare environments. Specific research activities have been carried out in the context of emergency wards and first aid environments (e.g., \cite{2006technology}). According to reported results about the procedures, interaction patterns and supporting systems, the main causes of delays, inefficiencies and medical errors can be ascribed to the lack of proper interaction between the medical staff and IT systems, which are, in turn, loosely integrated in healthcare workflows, leading to duplicated or suboptimal task allocation policies. In emergency departments, which presently represent the main access point for citizens to healthcare services, the medical staff operates under stress conditions in a rapidly evolving environments \cite{laxmisan2007multitasking}. Our work and initial effort can be broadly positioned in this context, where the introduction of multimodal interaction with vocal interface can lead to a significant benefits for both patients and clinicians, allowing to conduct the healthcare tasks in such environment easier and faster, and help medical staff while physically examine their patients in order to improve the overall performance. 
